Map as The Hidden Sensor: Fast Odometry-Based Global Localization

Accurate and robust global localization is essential to robotics applications. We propose a novel global localization method that employs the map traversability as a hidden observation. The resulting map-corrected odometry localization is able to provide an accurate belief tensor of the robot state. Our method can be used for blind robots in dark or highly reflective areas. In contrast to odometry drift in long-term, our method using only odometry and the map converges in longterm. Our method can also be integrated with other sensors to boost the localization performance. The algorithm does not have any initial state assumption and tracks all possible robot states at all times. Therefore, our method is global and is robust in the event of ambiguous observations. We parallel each step of our algorithm such that it can be performed in real-time (up to ~ 300 Hz) using GPU. We validate our algorithm in different publicly available floor-plans and show that it is able to converge to the ground truth fast while being robust to ambiguities.

==> probform.tex <==
\section{Problem Formulation}
The map of an indoor environment is given as $M$ where a pixel region $k$ is characterized as free $P(m_{free} \in M) = 0$ or occupied space $P(m_{occ} \in M) = 1$. The state of the robot at time $t$ is $x_t \in SE(2) $ that contains both position and orientation. Each pixel will represent a state of the robot and we assume an uniform distribution for each state $\hat{x}_t$ within a predefined region $k$.
\begin{equation}
    P(x_{k,t}) = |k|^{-1}\int_{k} P(\hat{x}_t) d\hat{x}_t
\end{equation}
where $|k|$ is the area of the region $k$.
The odometry motion at time $t$ is defined as $u_t$ such that the transitional probability from state $x_{t-1}$ to $x_t$ is given as $P(x_t | u_t, x_{t-1})$. For a discrete region $k$, the probability that the robot state is at location $k$ is given as 
\begin{equation}\label{eq:motion_update}
P(x_{k,t} | u_{1:t}) = \sum_{i \in M} P(x_{k,t} | u_t, x_{i,t-1}) P(x_{i,t-1})
\end{equation}

After updating the belief map with motion, we can then updated with the observation model $P(z_t | x_{k,t})$. The final belief at location $k$ is then given as
\begin{equation}\label{eq:sensor_update}
    P(x_{k,t} | u_{1:t}, z_t) = \eta P(z_t | x_{k,t}) P(x_{k,t} | u_{1:t})
\end{equation}
where $\eta$ is the normalization factor such that $\sum_{k}P(x_{k,t} | u_{1:t}, z_t) = 1$.
Therefore, each region $k$ in the final belief map $P(x_{k,t} | u_{1:t}, z_t) \in B_t$ can be estimated.
We also define the belief map ${P}(x_{k,t} | u_{1:t}) \in B_{u,t}$ that is only updated with the motion. 

In this paper, we assume the initial state of the robot is unknown and the only inputs are a set of odometry measurements and a map. In another words, the robot moves in the map blindly and tries to localize itself.

